Attacking Graph Convolutional Networks via Rewiring

Graph Neural Networks (GNNs) have boosted the performance of many graph related tasks such as node classification and graph classification. Recent researches show that graph neural networks are vulnerable to adversarial attacks, which deliberately add carefully created unnoticeable perturbation to the graph structure. The perturbation is usually created by adding/deleting a few edges, which might be noticeable even when the number of edges modified is small. In this paper, we propose a graph rewiring operation which affects the graph in a less noticeable way compared to adding/deleting edges. We then use reinforcement learning to learn the attack strategy based on the proposed rewiring operation. Experiments on real world graphs demonstrate the effectiveness of the proposed framework. To understand the proposed framework, we further analyze how its generated perturbation to the graph structure affects the output of the target model.

==> sections/theory.tex <==
\section{Propeties }\label{sec:theory}
\begin{itemize}
    \item Some general properties: degree; number of nodes; number of edges
    \item A graph can be fully characterized by its Laplacian matrix. The eigenvalue and eigenvectors are important information for the graph. The first few eigenpairs are especially important. 
    
    \item Some important graph measures are based on the eigenvalues 
\end{itemize}
In this section, we show that the rewiring operations can preserve important graph properties in a better way than directly adding and deleting edges. 


{\bf some simple properties we only need to include such as the number of edge, the number of nodes......, though the proof is straightforward.....}

We can show that the operation of rewiring to 2-hop neighbors will only ``slightly'' change the first few eigenvalues of the Laplacian matrix of the graph through matrix perturbation theory. 

Let $\lambda_i, {\bf \mu}_i$ be the ith eigen-pair (eigenvalue, eigenvector) of a symmetric matrix ${\bf A}$. Let $\Delta {\bf A}$ and $(\Delta \lambda_i, \Delta {\bf \mu}_i)$ denote the change in ${\bf A}$ and $\lambda_i, {\bf \mu}_i$ respectively. That is to say, that if the matrix ${\bf A}$ is modified to ${\bf A}+ \Delta{\bf A}$, the eigen-pair is changed to $({\lambda_i + \Delta \lambda_i, \mu_i + \Delta \mu_i})$. We have the following lemma.
\begin{lemma} \citep{stewart1990matrix}
Given a perturbation $\Delta {\bf A}$ to matrix ${\bf A}$, its eigenvalues can be updated by 
 $$\Delta \lambda_i = \mu_i^T \Delta {\bf A} \mu_i.$$ 
\end{lemma}\label{lemma:eigenvalue}


Now, let us consider the Laplacian matrix and measure how a perturbation of ``rewiring to 2-hop neighbors'' can affect the (first few) eigenvalues. let us denote the rewiring operation as $(a,b,c)$, which means, we remove the edge $(a,b)$ and add the edge $(a,c)$. Note here, $c$ is 2-hop neighbor of $a$.

The change of Laplacain matrix of the rewiring can be denoted as 
\begin{align}
    \Delta {\bf L}_{rewiring} = \Delta {\bf L}_{add} + \Delta {\bf L}_{remove}
\end{align}

So, the change of the eigenvalues of ${\bf L}$ can be described as follows
\begin{align*}
    \mu_i^T \Delta {\bf L}_{rewiring} \mu_i &= \mu_i^T \Delta {\bf L}_{remove} \mu_i + \mu_i^T \Delta {\bf L}_{add} \mu_i\\
    & = -\mu_i[a] ^2 - \mu_i[b]^2 + 2\mu_i[a] \mu_i[b] + \mu_i[a]^2 + \mu_i[c]^2 - 2\mu_i[a]\mu_i[c]\\
    &= \mu_i[c]^2 - \mu_i[b]^2 + 2\mu_i(\mu_i[b]-\mu_i[c])\\
    & = (2\mu_i[a] - \mu_i[c] -\mu_i[b])(\mu_i[b]-\mu_i[c])
\end{align*}
Ideally, the first few eigenvectors should be ``smooth'', which means that close nodes should have similar values, which could lead to ``small values'' of the change in eigenvalue we derived above. 



\subsection{aaa}
Let $\mathbf{P} = ReLU(\mathbf{A} \mathbf{X} \mathbf{W})$ and $\mathbf{Q} = ReLU(\mathbf{B} \mathbf{X} \mathbf{W})$, then $P_{ij} - Q_{ij}$ is given as
\begin{equation}
    P_{ij} - Q_{ij} = ReLU(\mathbf{a}^i \mathbf{X} \mathbf{w}_j) -  ReLU(\mathbf{b}^i \mathbf{X} \mathbf{w}_j)
\end{equation}
where $\mathbf{a}^i$ and $\mathbf{w}_j$ are the i-th row of $\mathbf{A}$ and $j$-th column of $\mathbf{B}$, respectively. Obviously, if $\mathbf{a}^i = \mathbf{b}^i$, then $P_{ij} - Q_{ij} = 0$. Thus, we are only interested in the case that $\mathbf{a}^i \ne \mathbf{b}^i$, i.e., rows that have actions of adding/deleting edges. In general there are four cases:
\begin{equation}
    P_{ij} - Q_{ij} =
			\left\{
   			\begin{array}{c}
   				\sum_{s,t} (A_{is} - B_{is}) \mathbf{X}_{st} \mathbf{W}_{tj}, \quad \text{if } \mathbf{a}^i \mathbf{X} \mathbf{w}_j > 0
\text{ and } \mathbf{b}^i \mathbf{X} \mathbf{w}_j > 0 \\
 			  	\sum_{s,t} A_{is} \mathbf{X}_{st} \mathbf{W}_{tj}, \quad\quad\quad \text{if } \mathbf{a}^i \mathbf{X} \mathbf{w}_j > 0
\text{ and } \mathbf{b}^i \mathbf{X} \mathbf{w}_j \le 0 \\
                \sum_{s,t} B_{is} \mathbf{X}_{st} \mathbf{W}_{tj}, \quad\quad\quad \text{if } \mathbf{a}^i \mathbf{X} \mathbf{w}_j \le 0
\text{ and } \mathbf{b}^i \mathbf{X} \mathbf{w}_j > 0 \\
                0, \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \text{if } \mathbf{a}^i \mathbf{X} \mathbf{w}_j \le 0
\text{ and } \mathbf{b}^i \mathbf{X} \mathbf{w}_j \le 0
   			\end{array}
  			\right.
\end{equation}

%\noindent{}\textbf{Case 1:} If $\mathbf{a}^i \mathbf{X} \mathbf{w}_j > 0$
%and $\mathbf{b}^i \mathbf{X} \mathbf{w}_j > 0$, then
%\begin{equation}
%    P_{ij} - Q_{ij} = (\mathbf{a}^i - \mathbf{b}^i) \mathbf{X} \mathbf{w}_j = \sum_{s,t} (A_{is} - B_{is}) \mathbf{X}_{st} \mathbf{W}_{tj}
%\end{equation}
%Suppose that $e_{iu}$ is rewired to $e_{iv}$, then the above equation becomes

\subsection{bbb}
Let $\mathbf{A} \in \{0,1\}^{n \times n}$ be the adjacency matrix. Assume that edge $e_{st}$ is added to $\mathbf{A}$. Then the new adjacency matrix $\tilde{\mathbf{A}} = \mathbf{A} + \Delta \mathbf{A}$, where $\Delta A_{ts}=1$, $\Delta A_{st}=1$ and all the other elements of $\Delta \mathbf{A}$ is 0. The embedding change can be written as
\begin{equation}
\begin{aligned}
    \|\tilde{\mathbf{A}}\mathbf{X} \mathbf{W} - \mathbf{A} \mathbf{X} \mathbf{W}\|_F^2 & = \sum_i  \sum_j (\sum_{k} \Delta A_{ik} (\mathbf{XW})_{kj})^2 \\
    & = \sum_j ((\mathbf{XW})_{tj})^2 + \sum_j (\mathbf{XW}_{tj})^2 \\
    & = \|(\mathbf{XW})[s,:]\|_2^2 + \|(\mathbf{XW})[t,:]\|_2^2
\end{aligned}
\end{equation}
The above analysis tells us the embedding change by adding one edge $e_{st}$ is simply $\|(\mathbf{XW})[s,:]\|_2^2 + \|(\mathbf{XW})[t,:]\|_2^2$. Suppose we randomly add an edge to the graph, then the embedding change is bounded as follows
\begin{equation}
\begin{aligned}
    \|\tilde{\mathbf{A}}\mathbf{X} \mathbf{W} - \mathbf{A} \mathbf{X} \mathbf{W}\|_F^2 & \ge \min_{st: e_{st} \ne \mathcal{E}} \|(\mathbf{XW})[s,:]\|_2^2 + \|(\mathbf{XW})[t,:]\|_2^2 \\
    \|\tilde{\mathbf{A}}\mathbf{X} \mathbf{W} - \mathbf{A} \mathbf{X} \mathbf{W}\|_F^2 & \le \max_{st: e_{st} \ne \mathcal{E}} \|(\mathbf{XW})[s,:]\|_2^2 + \|(\mathbf{XW})[t,:]\|_2^2
\end{aligned}
\end{equation}
